Enhancing Question Answering on Charts Through Effective Pre-training Tasks

To completely understand a document, the use of textual information is not enough. Understanding visual cues, such as layouts and charts, is also required. While the current state-of-the-art approaches for document understanding (both OCR-based and OCR-free) work well, a thorough analysis of their capabilities and limitations has not yet been performed. Therefore, in this work, we addresses the limitation of current VisualQA models when applied to charts and plots. To investigate shortcomings of the state-of-the-art models, we conduct a comprehensive behavioral analysis, using ChartQA as a case study. Our findings indicate that existing models particularly underperform in answering questions related to the chart's structural and visual context, as well as numerical information. To address these issues, we propose three simple pre-training tasks that enforce the existing model in terms of both structural-visual knowledge, as well as its understanding of numerical questions. We evaluate our pre-trained model (called MatCha-v2) on three chart datasets - both extractive and abstractive question datasets - and observe that it achieves an average improvement of 1.7% over the baseline model.

==> tables/checklist_results.tex <==
\begin{table*}[tb]
\tabprespace{}
  \small
  \centering
%   \resizebox{\columnwidth}{!}{
  \resizebox{\linewidth}{!}{
  \setlength{\tabcolsep}{3pt}
      \begin{tabular}{cm{4cm}rrrrrm{11cm}}
    \toprule
    
    \multicolumn{2}{c}{\multirow{2}{*}{\bfseries Template Type and Description}} &
    \multicolumn{5}{c}{\bf Failure Rate (\%)}  &
    \multicolumn{1}{c}{\multirow{2}{*}{\bf Example \& Expected answer}}\\
    \cmidrule(lr){3-7}
    &
    &
    \multicolumn{1}{c}{\matcha} &
    \multicolumn{1}{c}{\deplot} & 
    % &
    \\
    \midrule
    
    \bottomrule
  \end{tabular}
  }
  \vspace{-1mm}
  \caption{A selection of tests for the~\chartqa checklist. 
  \vspace{-2mm}
  } \label{tab:eg:chartqa}
\tabpostspace{}
\end{table*}

==> tables/datasets.tex <==
\begin{table}[]
\begin{tabular}{@{}llll@{}}
\toprule
% Dataset & \# Train   & \# Dev    & \# Test   \\ \midrule
% ChartQA & 28299      & 1920      & 2500      \\
% PlotQA  & 20,249,479 & 4,360,648 & 4,342,514 \\
% OpenCQA & -          &           &           \\ \bottomrule
Dataset & Chart       & \# of      & \# of    \\ 
 & types       & Charts     & QA pairs   \\ \midrule
ChartQA & Bar,         & ~800      & 2500      \\
 & Line         &       &       \\
% chart qa only include OWID numbers for QA and charts
PlotQA  & Bar, Line,        & ~224k & ~28.9m \\
        & Scatter           &       &        \\
OpenCQA & Bar, Scatter,     & ~7.7k &  ~7.7k         \\ 
        & Line, Area,    &           &           \\ 
        & Pie               &           &           \\ \bottomrule
\end{tabular}
\caption{\textbf{Dataset Details.} Statistics of the datasets along with relevant information such as the number of QA pairs and chart types.}
\label{tab:dataset_stats}
\end{table}

==> tables/model.tex <==
\begin{table}[]
\begin{tabular}{@{}lccc@{}}
\toprule
Model        & \# of params       & end-to-end \\ \bottomrule
MatCha       &  300M              & Yes \\ 
DePlot (+LLM) &  282M + O(LLM)     & No \\ \bottomrule
\end{tabular}
\caption{\textbf{Model Details.} Statistics of the modeling approaches along with relevant information such as the number of parameters.}
\label{tab:model_stats}
\end{table}

==> tables/pretraining_figure.tex <==
\begin{figure*}[]
\centering
\includegraphics[width=.95\textwidth]{images/pre-training_example.pdf}
\caption{The proposed pre-training procedures: Vi-Struct Pre-training and Statistics Pre-training}
\label{lab:pretraining}
\end{figure*}

